Observational causality by states and interaction type for scientific discovery

Causality plays a central role in understanding interactions between variables in complex systems. These systems often exhibit state-dependent causal relationships, where both the strength and direction of causality vary with the value of the interacting variables. In this work, we introduce a state-aware causal inference method that quantifies causality in terms of information gain about future states. The effectiveness of the proposed approach stems from two key features: its ability to characterize causal influence as a function of system state, and its capacity to distinguish between redundant and synergistic interactions. The method is validated across a range of benchmark cases in which the direction and strength of causality evolve in a prescribed manner with the state of the system. We further demonstrate the applicability of our approach in two real scenarios: the interaction between motions across scales in a turbulent boundary layer, and the Walker circulation phenomenon in tropical Pacific climate dynamics. Our results show that, without accounting for state-dependent causality as well as redundant and synergistic effects, traditional approaches to causal inference may lead to incomplete or misleading conclusions.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> preamble.tex <==
\usepackage[affil-it]{authblk}
\usepackage{titlesec} % For customizing section titles
\usepackage{setspace} % For adjusting line spacing
\usepackage[twoside,
            letterpaper,includeheadfoot,%
            layoutsize={8.125in,10.875in},%
            layouthoffset=0.1875in,%
            layoutvoffset=0.0625in,%
            left=38.5pt,%
            right=43pt,%
            top=43pt, % 10pt provided by headsep
            bottom=32pt,%
            headheight=0pt, % No Header
            headsep=10pt,%
            footskip=25pt,
            marginparwidth=38pt]{geometry}

\usepackage{lmodern} % Ensure Latin Modern Sans Serif is used
% \renewcommand{\familydefault}{\sfdefault}

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{xcolor}
% \usepackage{bm}
% \usepackage{amsbsy}
\usepackage{fixmath}
\usepackage{subcaption}
\usepackage{adjustbox}
\usepackage{pifont}
\usepackage{cancel}
\usepackage{url}

\definecolor{myc1}{HTML}{003049}
\definecolor{myc2}{HTML}{d62828}
\definecolor{myc3}{HTML}{f77f00}
\definecolor{myc4}{HTML}{6ca13b}

\definecolor{Q2}{HTML}{1f77b4}
\definecolor{Q1}{HTML}{ff7f0e}
\definecolor{Q3}{HTML}{2ca02c}

\definecolor{Q2}{HTML}{6ca13b}
\definecolor{Q1}{HTML}{6ca13b}
\definecolor{Q3}{HTML}{6ca13b}

\usepackage{tikz}
\usepackage{tikz-3dplot}
\usepackage{pgfplots}
\usetikzlibrary{decorations.markings,arrows.meta,calc,shapes,intersections,backgrounds,patterns.meta,bending,angles,decorations.pathreplacing,decorations.pathmorphing,pgfplots.colorbrewer,math}
\usepgfplotslibrary{fillbetween}
\usepackage{xifthen}
\usepackage[normalem]{ulem}
% \usepackage{pdflscape}
\usepackage{xcolor}
% \usepackage[export]{adjustbox}
% \usepackage{hyperref}

% \pgfplotsset{compat=1.12} % TikZ coordinates <-> axes coordinates
% \pgfplotsset{compat=1.12}

% Adjust the default font size and line spacing for the document
\AtBeginDocument{
  \fontsize{6pt}{10pt}\selectfont
  \setstretch{0.975}
}

% Customize section titles to be bold and use lmss
\titleformat*{\section}{\bfseries\fontfamily{lmss}\large\selectfont}
\titleformat*{\subsection}{\bfseries\fontfamily{lmss}\selectfont}
\titleformat*{\subsubsection}{\bfseries\fontfamily{lmss}\selectfont}

% Add 'S' prefix to figures, tables, and equations
\counterwithin{figure}{section}
\renewcommand{\thefigure}{S\arabic{figure}}
\counterwithin{table}{section}
\renewcommand{\thetable}{S\arabic{table}}
\counterwithin{equation}{section}
\renewcommand{\theequation}{S\arabic{equation}}

% Title, authors, and affiliations formatting
\usepackage{etoolbox} % Required for command redefinitions
\let\oldtitle\title
\renewcommand{\title}[1]{\oldtitle{{\fontfamily{lmss}\selectfont #1}}}
\let\oldauthor\author
\renewcommand{\author}[1]{\oldauthor{\large\fontfamily{lmss}\selectfont #1}}
\let\oldaffil\affil
\renewcommand{\affil}[1]{\oldaffil{\large\fontfamily{lmss}\selectfont #1}}

\newcommand{\cmark}{\ding{51}}% Checkmark
\newcommand{\xmark}{\ding{55}}% X mark

%----------------------------------------------------------------------
%----Helper code for dealing with external references----
% (by cyberSingularity at http://tex.stackexchange.com/a/69832/226)

\usepackage{xr}
% \usepackage[export]{adjustbox}
\makeatletter

\newcommand*{\addFileDependency}[1]{% argument=file name and extension
\typeout{(#1)}% latexmk will find this if $recorder=0
% however, in that case, it will ignore #1 if it is a .aux or 
% .pdf file etc and it exists! If it doesn't exist, it will appear 
% in the list of dependents regardless)
%
% Write the following if you want it to appear in \listfiles 
% --- although not really necessary and latexmk doesn't use this
%
\@addtofilelist{#1}
%
% latexmk will find this message if #1 doesn't exist (yet)
\IfFileExists{#1}{}{\typeout{No file #1.}}
}\makeatother

\newcommand*{\myexternaldocument}[1]{%
\externaldocument{#1}%
\addFileDependency{#1.tex}%
\addFileDependency{#1.aux}%
}
%------------End of helper code--------------

